Prediction Confidence from Neighbors

The inability of Machine Learning (ML) models to successfully extrapolate correct predictions from out-of-distribution (OoD) samples is a major hindrance to the application of ML in critical applications. Until the generalization ability of ML methods is improved it is necessary to keep humans in the loop. The need for human supervision can only be reduced if it is possible to determining a level of confidence in predictions, which can be used to either ask for human assistance or to abstain from making predictions. We show that feature space distance is a meaningful measure that can provide confidence in predictions. The distance between unseen samples and nearby training samples proves to be correlated to the prediction error of unseen samples. Depending on the acceptable degree of error, predictions can either be trusted or rejected based on the distance to training samples. %Additionally, a novelty threshold can be used to decide whether a sample is worth adding to the training set. This enables earlier and safer deployment of models in critical applications and is vital for deploying models under ever-changing conditions.

==> openended.tex <==
%\subsection{Open-ended Learning}
% open-ended learning, incremental learning
%Open-ended Learning or incremental learning addresses the problem that, in the real world, the distribution of data will change over time and thus it is likely to diverge from the training distribution.  train a new classifier for each new batch of data and weighting all previous classifiers according to their accuracy on recent samples~\cite{elwell2011incremental}.

%% open-ended learning %%
%"In this context, “open-ended” implies that the set of object categories to be learned is not known in advance, and the training instances are extracted from on-line experiences of a robot, and become gradually available over time, rather than being completely available at the beginning of the learning process."
%We don't know the true distribution. But can we make any assumptions that will be more or less universally true? e.g. that we should start with a uniform distribution and that the distribution should be adapted over time as more experience is collected.
%Incremental Learning methods are being proposed as a solution to the problem. However, non of the methods are widely used.

%Different types of changing distributions
%A typical assumption in machine learning is that the training and test data belong to the same distribution, that is often violated when a system is introduced in the field applications. ~\cite{DBLP:journals/corr/abs-1807-04950}
%DL in the wild~\cite{DBLP:journals/corr/abs-1807-04950} unforeseen samples are encountered, which results in unwanted outcomes. 


